SEAGLE - I: A pipeline for simulating and modeling strong lenses from cosmological hydrodynamic simulations

In this paper we introduce the SEAGLE (i.e. Simulating EAGLE LEnses) program, that approaches the study of galaxy formation through strong gravitational lensing, using a suite of high-resolution hydrodynamic simulations, Evolution and Assembly of GaLaxies and their Environments (EAGLE) project. We introduce the simulation and analysis pipeline and present the first set of results from our analysis of early-type galaxies. We identify and extract an ensemble of simulated lens galaxies and use the GLAMER ray-tracing lensing code to create mock lenses similar to those observed in the SLACS and SL2S surveys, using a range of source parameters and galaxy orientations, including observational effects such as the Point-Spread-Function (PSF), pixelization and noise levels, representative of single-orbit observations with the Hubble Space Telescope (HST) using the ACS-F814W filter. We subsequently model these mock lenses using the code LENSED, treating them in the same way as observed lenses. We also estimate the mass model parameters directly from the projected surface mass density of the simulated galaxy, using an identical mass model family. We perform a three-way comparison of all the measured quantities with real lenses. We find the average total density slope of EAGLE lenses, $t=2.26\; (0.25\; \rm{rms})$ to be higher than SL2S, $t=2.16$ or SLACS, $t=2.08$. We find a very strong correlation between the external shear ($\gamma$) and the complex ellipticity ($\epsilon$), with $\gamma \sim \epsilon/4$. This correlation indicates a degeneracy in the lens mass modeling. We also see a dispersion between lens modeling and direct fitting results, indicating systematical biases.

==> SEAGLE-I/implications.tex <==
\section{Implications on galaxy formation}\label{implications}
Analysis of simulated lenses from different scenarios are required to have a substantial evidence on the effects of different subgrid physics on the formation mechanisms of the galaxies. The calibrated simulations adopt identical initial conditions, enabling galaxies to be compared individually as well as statistically. SEAGLE II (Mukherjee et al. 2017b in prep.) will provide detailed analysis of the different formation scenarios to constrain the actual galaxy formation mechanisms that might be going in the lensing galaxies. 



==> SEAGLE-I/lensbasic.tex <==
\section{The lens equation}
\label{sec:basiclensing}

\begin{figure}

\includegraphics[width=.5\textwidth]{lensconfig}
	\caption{The geometry of gravitational lensing}

\end{figure}
The phenomenon of gravitational lensing is depicted in Fig.3.1 where a mass concentration at a distance $D_{\rm d}$ deflects the light rays from a source at a distance $D_{\rm s}$. The magnitude and direction of the bending of light is described by the deflection angle $ \hat{\alpha}$.
From the geometrical picture of gravitational lensing it is clear from the similar triangles and the small-angle approximation $\left( \sin \hat{\alpha} \approx \hat{\alpha} \approx \tan \hat{\alpha} \right)$,
\begin{equation}
\frac{\Big(\mathbold {\eta} + D_{\rm ds} \ \mathbold{ \hat{\alpha} (\xi)}\Big)}{D_{\rm s}}=\frac{\mathbold \xi}{D_{\rm d}}\ ,
\end{equation} 
where $D_{\rm s}, D_{\rm d}, D_{\rm ds}$ are angular diameter distances as shown in Fig.3.1. The above geometrical identity  can be rewritten as
\begin{equation}
\mathbold{\eta}= \frac{D_{\rm s}}{D_{\rm d}} \ {\mathbold \xi} - D_{\rm ds} \ \mathbold{ \hat{\alpha} (\xi)}\ .
\end{equation}
Using the angular coordinates defined by $\mathbold{\eta}= D_{\rm s} \mathbold{\beta}$ and $\mathbold{\xi}= D_{\rm d} \mathbold{\theta}$ we can write the equation as,
\begin{equation}
\mathbold {\beta}=\mathbold {\theta}-\frac{D_{\rm ds}}{D_{\rm s}} \ \mathbold {\hat{\alpha}} (D_{\rm d} \mathbold{\theta}) = \mathbold {\theta} - \mathbold{\alpha} \ ,
\end{equation}
where we have introduced the scaled deflection angle $\mathbold{ \alpha}=\frac{D_{\rm ds}}{D_{\rm s}} \ \mathbold {\hat{\alpha}} (D_{\rm d} \mathbold{\theta})$.\\
\ \\
The above equation is called the lens equation. So, a source with true angular position $\mathbold \beta$ will be seen by observer at angular positions $\mathbold \theta$ which may have different values giving rise to multiple images of a single source. The scaled deflection angle can be written in terms of the surface mass density as follows:
\begin{equation}
{\mathbold \alpha(\theta)}=\frac{1}{\pi} \ \int_{\mathbold \mathbb{R}^2}  d^2 {\theta}^{'} \ \kappa ({\mathbold \theta}^{'}) \  \frac{\mathbold{\theta}-\mathbold{{\theta}^{'}}}{|\mathbold{\theta}-\mathbold{{\theta}^{'}}|^2} \ ,
\end{equation}
where the \em convergence \em or dimensionless surface mass density is defined as
\begin{equation}
\kappa ({\mathbold \theta}) = \frac{\Sigma (D_{\rm d} \mathbold \theta)}{\Sigma_{\rm cr}} \qquad ; \qquad \Sigma_{\rm cr}=\frac{c^2}{4\pi G} \frac{D_{\rm s}}{D_{\rm d} \ D_{\rm ds}} \ .
\end{equation}
Here the \em critical surface mass density \em $\Sigma_{\rm cr}$ gives us a limit of strong or weak lensing. If $\kappa \geq 1$ or $\Sigma \geq \Sigma_{\rm cr}$ we can get multiple images for a single source.
\ \\
Now using the mathematical identity $\nabla  \ln |{\mathbold \theta}| \equiv {\mathbold \theta}/|{\mathbold \theta}|^2$ we can write the scaled deflection angle as a gradient of a scalar potential,
\begin{equation}
{\mathbold \alpha}=\nabla \psi \ ,
\end{equation}
where the lensing deflection potential is defined as,
\begin{equation}
\psi({\mathbold \theta})=\frac{1}{\pi} \int_{\mathbold \mathbb{R}^2} d^2 {\theta}^{'} \ \kappa (\mathbold{{\theta}^{'}}) \ln |\mathbold {\theta}-\mathbold {\theta^{'}}|.
\end{equation}
Also we may write the Poisson's equation in two dimensions by using the identity $\nabla^2  \ln |\mathbold {\theta}| \equiv 2\pi \delta ({\mathbold \theta})$ where $\delta({\mathbold \theta}) $ denotes Dirac delta function:
\begin{equation}
\nabla^2  \psi = 2 \kappa \ .
\end{equation}



